STITCH: Augmented Dexterity for Suture Throws Including Thread Coordination and Handoffs

We present STITCH: an augmented dexterity pipeline that performs Suture Throws Including Thread Coordination and Handoffs. STITCH iteratively performs needle insertion, thread sweeping, needle extraction, suture cinching, needle handover, and needle pose correction with failure recovery policies. We introduce a novel visual 6D needle pose estimation framework using a stereo camera pair and new suturing motion primitives. We compare STITCH to baselines, including a proprioception-only and a policy without visual servoing. In physical experiments across 15 trials, STITCH achieves an average of 2.93 sutures without human intervention and 4.47 sutures with human intervention. See https://sites.google.com/berkeley.edu/stitch for code and supplemental materials.

==> tables/experimental_results.tex <==

\begin{table}[htbp!]
\caption{\label{experiment-table}STITCH Experimental Results for \textit{n} Consecutive Suture Throws.}
\centering
{\begin{tabular}{cccc}
\toprule[1pt]
\textbf{\# of Throws} & \textbf{Success Rate} & \textbf{Average Time} & \textbf{\# of Trials} \\
 & (\%) & (sec) & (\#) \\
\midrule[0.1pt]
\textbf{1}  & 100 & 10 & 50 \\
\textbf{2}  & 100 & 10 & 50 \\
\textbf{3}  & 100 & 10 & 50 \\
\textbf{4}  & 100 & 10 & 50 \\
\textbf{5}  & 100 & 10 & 50 \\
\textbf{6+} & 100 & 10 & 50 \\
\bottomrule[1pt]
\end{tabular}}

\end{table}
